Unicyclic Graphs with equal Laplacian Energy

We introduce a new operation on a class of graphs with the property that the Laplacian eigenvalues of the input and output graphs are related. Based on this operation, we obtain a family of order (square root of n) noncospectral unicyclic graphs on n vertices with the same Laplacian energy.

==> ref.tex <==
\begin{thebibliography}{99}

\bibitem{Brobook} Brouwer, Andries E.  and Haemers, Willem H., \emph{Spectra of graphs}, Springer, 2012.

\bibitem{FHRT11} Fritscher, E., Hoppen, C., Rocha, I., and Trevisan, V. On the sum of the laplacian eigenvalues of
a tree. Linear Algebra and its Applications 435 (2011), 371-399.

\bibitem{G78} Gutman, I. The energy of a graph. Ber. Math.-Statist. Sekt. Forschungszentrum Graz 103 (1978), 1-22.

\bibitem{GZ06} Gutman, I., and Zhou, B. Laplacian energy of a graph. Linear Algebra and its Applications 414 (2006),
29-37.

\bibitem{JT11} Jacobs, D. P., and Trevisan, V. Locating the eigenvalues of trees. Linear Algebra and its Applications
434 (2011), 81-88.

\bibitem{LS}  Li, C.-K., and So, W. Graphs equienergetic with edge-deleted subgraphs. Linear and Multilinear Algebra
57, 7 (2009), 683-693.

\bibitem{Ram2004} Ramane, H. S., Walikar, H. B., Rao, S. B., Acharya, B. D., Hampiholi, P. R., Jog, S. R., and
Gutman, I. Equienergetic graphs. Kragujevac Journal of Mathematics 26 (2004), 5-13.

\bibitem{Ste09} Stevanovic, D. Large sets of noncospectral graphs with equal Laplacian energy. MATCH Commun. Math.
Comput. Chem. 61, 2 (2009), 463-470.

\bibitem{yueh} Yueh, W.-C. Eigenvalues of several tridiagonal matrices. Applied Mathematics E-notes 5 (2005), 66-74.
\end{thebibliography}
